PPL-MCTS: Constrained Textual Generation Through Discriminator-Guided MCTS Decoding

Large language models (LM) based on Transformers allow to generate plausible long texts. In this paper, we explore how this generation can be further controlled at decoding time to satisfy certain constraints (e.g. being non-toxic, conveying certain emotions, using a specific writing style, etc.) without fine-tuning the LM. Precisely, we formalize constrained generation as a tree exploration process guided by a discriminator that indicates how well the associated sequence respects the constraint. This approach, in addition to being easier and cheaper to train than fine-tuning the LM, allows to apply the constraint more finely and dynamically. We propose several original methods to search this generation tree, notably the Monte Carlo Tree Search (MCTS) which provides theoretical guarantees on the search efficiency, but also simpler methods based on re-ranking a pool of diverse sequences using the discriminator scores. These methods are evaluated, with automatic and human-based metrics, on two types of constraints and languages: review polarity and emotion control in French and English. We show that discriminator-guided MCTS decoding achieves state-of-the-art results without having to tune the language model, in both tasks and languages. We also demonstrate that other proposed decoding methods based on re-ranking can be really effective when diversity among the generated propositions is encouraged.

==> content/background.tex <==
\section{Background}
\label{sec:background}

\paragraph{Text generation}
Language modeling estimates the probability distribution of sequences of symbols $x_1, x_2, \cdots, x_T$ (most often \textit{tokens}) taken from a vocabulary $\mathcal{V}$, with variable lengths $T$.
Most commonly, the probability of one sample $x$ (also called \textit{likelihood}) is defined as the joint probabilities over each of its tokens, which can be factorized using the chain rule: $p(x_{1:T})=\prod_{t=1}^{T} p(x_{t} \mid x_{1:t-1})$.

Given a training set %$\mathcal S$ % plus utilisé ensuite
of texts, a LM can be trained by optimizing weights $\theta$ of a neural network which outputs a probability distribution over the dictionary for the next token given the input ones, i.e  $p_\theta(x_t \mid x_{1:t-1})$ at a given time step $t$. 
%This training can be done by using the cross-entropy between the output probabilities and the one-hot representation of the ground-truth next token, in order to maximize the log-likelihood of the set of token sequences contained in our samples.
This allows to create an auto-regressive LM that can generate sequences by iteratively using those distributions to emit a token $x_t$, and append it to the context $x_{1:t-1}$ for the next iteration. The generation process --or \textit{decoding}-- is often started using a small initial sequence: the \textit{prompt}.


\paragraph{Decoding methods.}
%Generation requires to choose a token $x_t$ that should be appended to $x_{1:t-1}$.
However, how to choose a token $x_t$ so that the final sequence has the highest possible likelihood is still an open problem. This is mainly due to the size of the search space, since for a sequence of length $T$ and a vocabulary of size $\vert \mathcal{V} \vert$ (often being tens of thousand), the space has a size of  $\vert \mathcal{V} \vert^T$, making an exact search intractable. 
Several search methods have been proposed to alleviate this issue; a naive one is the \textit{greedy search} where the most probable token is picked at each step. 
A neural LM predicting logits $z_{1:\vert \mathcal{V} \vert}$ over the vocabulary, the probability of sampling the i\textsuperscript{th} token at time step $t$ is computed by applying softmax, usually with temperature $\tau$ (a high $\tau$ flattens the distribution): 
\begin{equation}
\label{eqn:sampling_prob}
%\pi_{\tau}(t)=p_\theta(s_t \mid s_{1}, \ldots, s_{t-1})=\frac{\exp \left(z(t) /\tau )\right.}{\sum_{v} \exp \left(z(v) /\tau )\right.
p_\theta(x_i \mid x_{1:t-1})=\frac{\exp \left(z_i /\tau )\right.}{\sum_{v} \exp \left(z_v /\tau )\right.}
\end{equation}


In order not to miss a more probable sequence which starts with a token having a lower probability, \textit{beam search}~\citep{dept._2018} explores the $k$ most probable sequences at each generation step.
%\ac{en fait, on explore jusqu'à une petite profondeur en gardant les $k$ plus probables à chaque fois qu'on descend. Mais pour une étape de génération, on a qu'un token choisi}\VC{j'ai légérement changé la formulation, ça va comme ça ?} 
It should be noted that these search methods are highly biased towards samples that have a high likelihood \textit{in the beginning}, which does not guarantee to find the sequence with the highest possible likelihood. Moreover, they tend to generate redundant texts; thus, \textit{top-k sampling}~\citep{DBLP:conf/acl/LewisDF18} samples the next token from the $k$ most probable next tokens to introduce variance. However, $k$ is fixed and the $k$\textsuperscript{th} token may have a very low probability (and therefore be off-topic). To improve upon this method, \textit{nucleus sampling}~\citep{DBLP:conf/iclr/HoltzmanBDFC20} (or \textit{top-p sampling}) is used to sample from the smallest set of tokens that have a cumulative probability higher than $p$. 
Finally, \textit{beam sampling}~\citep{DBLP:conf/iclr/CacciaCFLPC20} consists in a mix of beam search and sampling. $k$ tokens are first sampled using the LM distribution and, for each one, $k$ more tokens are then sampled, leading to $k^2$ beams in which only the $k$ most probable are kept. This process is repeated until each beam is finished. 
%\ac{C'est bon si on définit correctement la beam search au dessus. Peut être remplacer le "at the next timestep" par and $k$ more tokens are then sampled for each of these tokens. ça mélange moins le timestep de génération et d'exploration des beams} --> \VC{j'ai modifié, ça devrait être OK}

\paragraph{Tuning a constrained LM.}
As the LM only models $p_{\theta}(x)$, adding a constraint to guide the generation is not straightforward. The simplest way of applying a constraint to generations is to directly train a specific model $\theta_c$ on texts that belong to a class $c$ satisfying the constraint, thus modeling $p_{\theta_c}(x)$. However, this approach leads to train one specific LM for each constraint, resulting in several models. The idea of constrained textual generation as we aim in this paper is rather to model $p_{\theta}(x\mid c)$ with only one LM; hence, training is done once and the same $\theta$ is used for every constraint.

\paragraph{Discriminator-guided generation.} 
To avoid the computational cost of fine-tuning large LMs, some methods aim at controlling the generation only at decoding time. The general idea of discriminator-guided generation is to combine a disciminator $D$ with a generative LM.
Contrasting with the implicit application of constraint in tuned-models, the discriminator $D$ explicitly models the constraint by calculating the probability $p_{D}(c \mid x)$ of the sequence $x$ to satisfy the constraint $c$. This probability is directly related to $p(x\mid c)$ through Bayes' rule : $ p(x\mid c) \propto p_{D}(c \mid x) p_\theta(x)  $
%\begin{equation}
%\label{eqn:bayes}    
% p(x\mid c) \propto p_{D}(c \mid x) p_\theta(x)  
%\end{equation}

%The general idea of discriminator-guided generation is to plug a disciminator $D$ with a generative LM and to sample from the resulting: \ewa{A revoir : utilisation du terme "sampling" - utilisation de $p_{D}(c \mid x)$ de differente facons, notamment pour l'estimation de $p(x\mid c)$}

%One way to explicitly model it is to apply the Bayes' rule to the conditional probability : 
%\begin{equation}
%\label{eqn:bayes}
%p(x\mid c) = \frac{p(c \mid x)p(x)}{p(c)}
%\end{equation}
%where the prior $p(c)$ is the same for every sequence, $p(x)$ is the likelihood of the sequence $x$ given by the language model, while $p(c \mid x)$ is the probability of the sequence $x$ satisfying the constraint that can be approximated using a classifier trained to verify if a sequence satisfy the constraint or not. Such classifiers are easier to train than a LM and any additional constraint can be defined a posteriori without tuning the LM, only by training another classifier.

With this definition, finding the sequence that maximizes $p(x\mid c)$, consists in finding a sequence that is both well written (high LM likelihood) and that satisfies the constraint (high classification probability).
Yet, as previously mentioned, finding the sequence with the highest likelihood is not simple. Adding the constraint makes the process even more complicated since the most probable sequences might not satisfy the constraint, making heuristics used in traditional search methods even worse. Even if the discriminator is trained with inputs of variable lengths, its output probabilities become necessarily more meaningful as the sequence grows and might only be trustable to guide the search when the sequence is (nearly) finished, leading to similar problems as with likelihood. Thus, to achieve good constrained generation, one needs to find efficient ways of exploring this huge search space.


